TopoLines: Topological Smoothing for Line Charts

Line charts are commonly used to visualize a series of data values. When the data are noisy, smoothing is applied to make the signal more apparent. Conventional methods used to smooth line charts, e.g., using subsampling or filters, such as median, Gaussian, or low-pass, each optimize for different properties of the data. The properties generally do not include retaining peaks (i.e., local minima and maxima) in the data, which is an important feature for certain visual analytics tasks. We present TopoLines, a method for smoothing line charts using techniques from Topological Data Analysis. The design goal of TopoLines is to maintain prominent peaks in the data while minimizing any residual error. We evaluate TopoLines for 2 visual analytics tasks by comparing to 5 popular line smoothing methods with data from 4 application domains.

==> sec-related.tex <==



\section{Prior Work on Perception of Line Charts}


%~\cite{} and contour trees in general~\cite{}



Prior research has investigated how line chart visualizations affect user preference and ability. Techniques that optimize for graphical perception~\cite{1986tufte, 2005horizon, 2009heer} have been shown to improve both the accuracy and effectiveness for understanding line chart data~\cite{2010javed, 2016arbesser, 2019gogolou}. 
%Visualization techniques for line charts . 
For example, Javed et al.\ evaluated the effectiveness of line charts by testing users on their ability to perform comparison, slope, and discrimination tasks for each line chart technique. The results showed that, when comparing line charts using small multiples, horizon graphs, stacked graphs, and braided graphs, user performance varied depending on the data being displayed using separate or shared-space charts during analysis~\cite{2010javed}.  

Recent work has also been done to evaluate the influence of aspect ratio~\cite{2018aspectratio}, visual complexity~\cite{2018entropy}, and user interaction~\cite{2016adnan} with line charts. Wang et al.\ provided a robust selection method to recommend aspect ratios in line charts using the resultant vector and local
orientation resolution~\cite{2018aspectratio}. Ryan et al.\ proposed a technique to quantitatively measure the visual complexity in line charts using Pixel Approximate Entropy (PAE)~\cite{2018entropy}. Adnan et al.\ conducted graphical perception study to measure the effectiveness of interaction during the analysis of time series data~\cite{2016adnan}.

Although line charts are a common method for visualizing one dimensional data~\cite{1989kosslyn}, extensive studies have been completed to determine their effectiveness compared to other chart types. One study confirmed the tendency of users to associate bar charts with discrete entities and line charts with trends~\cite{Zacks1999BarsAL}. A more recent study explored this hypothesis further in a multi-chart experiment~\cite{2018saket}. They found that line charts are significantly more accurate than other charts for correlation and distribution tasks, thus, line charts are best for tasks requiring finding correlations. Finally, Wang et al.\ provided a method to automatically select an appropriate chart (line chart vs.\ scatter plot) when visualizing time series data~\cite{2018autochart}. 

Other line chart visualization challenges that have been investigated include accounting for user performance when there is missing data~\cite{2005eaton, 2012templ, 2018szafir}. For example, Song et al.\ demonstrated the different design choices that should be leveraged for line charts and bar graphs when estimating averages and trends that are missing values~\cite{2018szafir}. 


